Exploiting Rich Textual User-Product Context for Improving Sentiment Analysis

User and product information associated with a review is useful for sentiment polarity prediction. Typical approaches incorporating such information focus on modeling users and products as implicitly learned representation vectors. Most do not exploit the potential of historical reviews, or those that currently do require unnecessary modifications to model architecture or do not make full use of user/product associations. The contribution of this work is twofold: i) a method to explicitly employ historical reviews belonging to the same user/product to initialize representations, and ii) efficient incorporation of textual associations between users and products via a user-product cross-context module. Experiments on IMDb, Yelp-2013 and Yelp-2014 benchmarks show that our approach substantially outperforms previous state-of-the-art. Since we employ BERT-base as the encoder, we additionally provide experiments in which our approach performs well with Span-BERT and Longformer. Furthermore, experiments where the reviews of each user/product in the training data are downsampled demonstrate the effectiveness of our approach under a low-resource setting.

==> 6-Acknowledgement.tex <==
\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> Tables/tbl-01-stats.tex <==
\begin{tabular}{lrrccccc}
\toprule
    Datasets  & \multicolumn{1}{c}{Classes} & \multicolumn{1}{c}{Documents}  & Users & Products  & Docs/User & Docs/Product  & Words/Doc\\
    \midrule
    IMDB      &      1--10 &  84,919 & 1,310 & 1,635 & 64.82 & 51.94 & 394.6  \\
    Yelp-2013 &       1--5 &  78,966 & 1,631 & 1,633 & 48.42 & 48.36 & 189.3  \\
    Yelp-2014 &       1--5 & 231,163 & 4,818 & 4,194 & 47.97 & 55.11 & 196.9 \\
    \bottomrule
\end{tabular}%

==> Tables/tbl-05-cases-full-text.tex <==
\begin{tabular}{p{11cm}p{3cm}}
    \toprule
     Review & Label \\
     
    \midrule
    
Took travis here for one of our first dates and just love cibo. It 's situated in a home from 1913 and has colored lights wrapped all around the trees. You can either sit inside or on the gorgeous patio. Brick oven pizza and cheese plates offered here and it 's definitely a place for a cool date. & VP~(\cmark)  \\
\hline
a great sushi bar owned and operated by maggie and toshi who are both japanese. their product is always consistent and they always have a few good specials. service is great and the staff is very friendly and cheerful. value is really good particularly within their happy hour menu. our kids love it and they are always spoiled rotten by maggie and toshi so it is their favorite place. lastly we did a sake tasting there a few weeks ago and really had a great time. we all sat family style int he middle of the restaurant and got to experience some really interesting rice wines. we had a blast. great place & P~(\cmark)  \\

\hline

well , i was disappointed. i was expecting this one to be a jazzed up container store. but ... it was just average. i used to visit container store in houston near the galleria. it has a nice selection of things. people are always ready to help etc.. but , this one has an aloof sort of customer service crowd. they say nice things about your kid but do not offer to help. hmm ... i have seen similar things they were selling at ikea. the quality did seem a little better than ikea but if you are buying a laundry room shelf for your laundry detergent ... who the hell cares. its a shelf !  does n't matter if it has 15 coats of paint on the metal or 2 coats. i found one of those sistema lunch boxes that i have been looking for over here and it was on sale. will i go back ?  probably not. too far out for me , plus i like ikea better & Ne~(\cmark)  \\

\hline
love that they have vegan options , love that they are educated about gmo 's , food allergies , etc. and , i love their raw burger , well , i used to , i had it tonight and it was hard , like really hard. it used to be delicious !!!  i picked up my food to go and waited quite a bit before anyone even said hello , or took my order. i noticed a couple of customers walk up to the bar to ask for service , one i know wanted more peanut sauce. before i got my food a mother and son had walked out and they were both shaking their heads. it felt uncomfortable there. i was there a couple of months ago for lunch , had the same uncomfortable feeling but the food was great. and , several months ago i was there with my boyfriend on a friday night and everything was good , i do n't know what 's going on. i will give it a little bit before i return , if i return , i really do applaud the owners of their concept especially on the gmo issue .  & N~(\cmark)  \\ % neural models is difficult to understand the term gmo


\hline
Unfortunately tonight was the last night this location was open. The only two locations left in the valley are desert ridge and arrowhead. Please support them.  & VP~(\cmark)  \\ 

        
        
    
    
    \bottomrule
    \end{tabular}%

==> Tables/tbl-05b-cases.tex <==
\begin{tabular}{cp{15cm}cccccccccccccccccccccccccccccccccc}
    %\toprule
   %  Review \\%& Vanilla BERT & IUPC & MA-BERT & Ours \\
     
    %\midrule
    (a) & \textit{Took travis here for one of our first dates and just love cibo. It 's situated in a home from 1913 and has colored lights wrapped all around the trees. You can either sit inside or on the gorgeous patio. Brick oven pizza and cheese plates offered here and it 's definitely a place for a cool date.} (VP)\\
    
%...... Brick oven pizza and cheese plates offered here and it's definitely a place for a cool date. & VP~(\cmark)  & VP~(\cmark)  & VP~(\cmark) & VP~(\cmark)  \\
%\hline
(b) &  \textit{a great sushi bar owned and operated by maggie and toshi who are both japanese. their product is always consistent and they always have a few good specials. service is great and the staff is very friendly and cheerful. value is really good particularly within their happy hour menu. our kids love it and they are always spoiled rotten by maggie and toshi so it is their favorite place. lastly we did a sake tasting there a few weeks ago and really had a great time. we all sat family style int he middle of the restaurant and got to experience some really interesting rice wines. we had a blast. great place } (P)\\
%...... Service is great and the staff is very friendly and cheerful. Value is really good particularly within their happy hour menu ...... Great place. & VP~(\xmark)  & P~(\cmark)  & P~(\cmark) & P~(\cmark)  \\

%\hline
(c) &  \textit{well , i was disappointed. i was expecting this one to be a jazzed up container store. but ... it was just average. i used to visit container store in houston near the galleria. it has a nice selection of things. people are always ready to help etc.. but , this one has an aloof sort of customer service crowd. they say nice things about your kid but do not offer to help. hmm ... i have seen similar things they were selling at ikea. the quality did seem a little better than ikea but if you are buying a laundry room shelf for your laundry detergent ... who the hell cares. its a shelf !  does n't matter if it has 15 coats of paint on the metal or 2 coats. i found one of those sistema lunch boxes that i have been looking for over here and it was on sale. will i go back ?  probably not. too far out for me , plus i like ikea better} (Ne) \\

%I was disappointed ....... They say nice things about your kid but do not offer to help . Will I go back ?  Probably not ...... & VN~(\xmark)  & N~(\xmark)  & VN~(\xmark) & Ne~(\cmark)  \\
% COMMENTING OUT SINCE THE INTERPRETATION IN THE TEXT IS INCORRECT
% THE GMO PART IS THE POSITIVE PART OF THE REVIEW NOT THE NEGATIVE ONE (JF)
%\hline
%Love that they have vegan options , love that they are educated about GMO's ...... I will give it a little bit before I return , if I return , I really do applaud the owners of their concept especially on the GMO issue.  & VP~(\xmark)  & P~(\xmark)  & P~(\xmark) & N~(\cmark)  \\ % neural models is difficult to understand the term gmo

%\hline
(d) &  \textit{Unfortunately tonight was the last night this location was open. The only two locations left in the valley are desert ridge and arrowhead. Please support them.} (VP)\\\\

%Unfortunately tonight was the last night this location was open. The only two locations left in the valley are desert ridge and arrowhead. Please support them.  & Ne~(\xmark)  & N~(\xmark)  & VN~(\xmark) & N~(\xmark)  \\ 
%\midrule
       \end{tabular}
       \begin{tabular}{ccccc}
       \toprule
     Review & Vanilla BERT & IUPC & MA-BERT & Ours \\
     \midrule
     (a) & VP~(\cmark)  & VP~(\cmark)  & VP~(\cmark) & VP~(\cmark)\\
     (b) & VP~(\xmark)  & P~(\cmark)  & P~(\cmark) & P~(\cmark)  \\
     (c) & VN~(\xmark)  & N~(\xmark)  & VN~(\xmark) & Ne~(\cmark) \\
     (d) & Ne~(\xmark)  & N~(\xmark)  & VN~(\xmark) & N~(\xmark) \\         
    
    
    \bottomrule
    \end{tabular}%
